Model-Based and Graph-Based Priors for Group Testing

The goal of the group testing problem is to identify a set of defective items within a larger set of items, using suitably-designed tests whose outcomes indicate whether any defective item is present. In this paper, we study how the number of tests can be significantly decreased by leveraging the structural dependencies between the items, i.e., by incorporating prior information. To do so, we pursue two different perspectives: (i) As a generalization of the uniform combinatorial prior, we consider the case that the defective set is uniform over a \emph{subset} of all possible sets of a given size, and study how this impacts the information-theoretic limits on the number of tests for approximate recovery; (ii) As a generalization of the i.i.d.~prior, we introduce a new class of priors based on the Ising model, where the associated graph represents interactions between items. We show that this naturally leads to an Integer Quadratic Program decoder, which can be converted to an Integer Linear Program and/or relaxed to a non-integer variant for improved computational complexity, while maintaining strong empirical recovery performance.

==> Block_graphs_with_finite_edge_strength.tex <==
\subsection{Block graphs with finite edge strength}
We consider the scenario where the $n$ items have the following structure: a block graph with finite edge strength $\lambda$, i.e., the $n$ items are arranged in $n/q$ groups of size $q$, and the edge count of each  block/group can take any integer value from 0 to $\binom{q}{2}$.

The the edge count of each block (of $q$ vertices) follows the random graph model $G(q, p)$ where $p = 1 - \mathrm{exp}(- \lambda)$ \textcolor{red}{??} is the edge probability.
Each possible edge can be viewed as a Bernoulli random variable $X$ with $\mathbb{P}(1) = p$.
And so, for the $n$ items/vertices, the interactions can be viewed as $(n/q) \binom{q}{2}$  i.i.d.  Bernoulli random variable with $\mathbb{P}(1) = p$.

It follows that for $p \neq 0.5$, the typical set consists of all possible such block graphs whose number of edges equals the expected value, i.e., $(n/q) \cdot \binom{q}{2} \cdot p$.
By the stars and bars counting technique, the number of such graphs is the coefficient of $X^{(n/q) \cdot \binom{q}{2} \cdot p}$ in the polynomial 
\[
    \left(1+X + \dotsi + X^{\binom{q}{2}}\right)^{n/q}. 
        % \left( \frac{1- X^{\binom{q}{2}+1}}{} \right)
\]
By \cite{554237}, this can be written as the following sum
\[
    \sum_{i=\lceil\frac{X^{(n/q) \cdot \binom{q}{2} \cdot p} + n/q}{\binom{q}{2}+1}\rceil}^{n/q}
  (-1)^{n/q-i}\binom{n/q}{i} \binom{i(\binom{q}{2}+1)-1-(n/q) \cdot \binom{q}{2} \cdot p}{n/q-1}
\]

% Suppose the Ising model admits a typical set $\mathcal{S}_{\text{typ}}^{\lambda}$ of supports,  i.e., the real support $S$ satisfies $\mathbb{P}[S \in \mathcal{S}_{\text{typ}}^{\lambda}] \to 1$ as 
% the number of tests $t \to \infty$.





==> Saved.tex <==

\section{EXISTING LP DERIVATION}

Consider $P(u_{j}=1)=p$, where $p < 0.5$, and $P(u_{j}=0)=1-p$, for $j \in V$. Also consider that each outcome $Y_i$ is flipped with equal probability $\rho$. Then in the noisy setting the posterior probability $P(\uv|\mathsf{X},\Yv)$ is given as
\begin{equation}
    \begin{aligned}
        P(\uv|\mathsf{X},\Yv) &= \frac{P(\uv,\Yv|\mathsf{X})}{P(\Yv|\mathsf{X})} \\
        &\propto P(\uv)P(\Yv|\mathsf{X}) \\ 
        &= \prod_{j=1}^{n} P(u_j) \prod_{i=1}^{t} P(Y_{i}|\mathbf{X}_{i}) \\ 
        &= p^{\sum_{j=1}^{n} u_{j}}(1-p)^{n-\sum_{j=1}^{n} u_{j}}\rho^{\sum_{i=1}^{T} \xi_{i}}(1-\rho)^{T-\sum_{i=1}^{T} \xi_{i}} \\
        &\propto \big(\frac{p}{1-p}\big)^{\sum_{j=1}^{n} u_{j}} \big(\frac{\rho}{1-\rho}\big)^{\sum_{i=1}^{T} \xi_{i}},
    \end{aligned}
\end{equation}
where $\sum_{j=1}^{n} u_{j}$ is the number of defective items and $\sum_{i=1}^{T} \xi_{i} $ is the number of flipped tests, also known as the Hamming distance between the output $\Yv$ and the expected output that one would get if there were no noise. The estimated $\hat{\uv}$ and $\hat{\boldsymbol{\xi}}$ obtained through Maximum A Posterior MAP decoding are given as:
\begin{equation}
    \begin{aligned}
        \hat{\uv},\hat{\boldsymbol{\xi}} = &\argmax_{\uv,\boldsymbol{\xi}} P(\uv|\mathsf{X},\Yv) \\
        =&\argmax_{\uv,\boldsymbol{\xi}} \big(\frac{p}{1-p}\big)^{\sum_{j=1}^{n} u_{j}} \big(\frac{\rho}{1-\rho}\big)^{\sum_{i=1}^{t} \xi_{i}} \\
        =&\argmax_{\uv,\boldsymbol{\xi}} \sum_{j=1}^{n} u_{j}\log\big(\frac{p}{1-p}\big) + \sum_{i=1}^{t} \xi_{i}\log\big(\frac{\rho}{1-\rho}\big) \\
        =&\argmin_{\uv,\boldsymbol{\xi}} \sum_{j=1}^{n} u_{j} + \frac{\log\big(\frac{\rho}{1-\rho}\big)}{\log\big(\frac{p}{1-p}\big)}\sum_{i=1}^{t} \xi_{i},
    \end{aligned}
    \label{lp_log}
\end{equation}
where $\frac{\log\big(\frac{\rho}{1-\rho}\big)}{\log\big(\frac{p}{1-p}\big)}$ is the value set for $\eta$.

Similarly, when there is no noise, we have $P(Y_{i}|\mathbf{X}_{i})=1$ for $i \in \{1, \dots, t\}$ and the posterior probability $P(\uv|\mathsf{X},\Yv)$ is simplified as
\begin{equation}
    \begin{aligned}
        P(\uv|\mathsf{X},\Yv) &= \frac{P(\uv,\Yv|\mathsf{X})}{P(\Yv|\mathsf{X})} \\
        &\propto  \prod_{j=1}^{n} P(u_j) \prod_{i=1}^{T} P(Y_{i}|\mathbf{X}_{i}) \\ 
        &= p^{\sum_{j=1}^{n} u_{j}}(1-p)^{n-\sum_{j=1}^{n} u_{j}} \times 1 \\
        &\propto \big(\frac{p}{1-p}\big)^{\sum_{j=1}^{n} u_{j}},
    \end{aligned}
\end{equation}
where $\sum_{j=1}^{n} u_{j}$ is the number of defective items given by the probabilistic model. By applying MAP again we get the estimated $\hat{\uv}$ as
\begin{equation}
    \begin{aligned}
        \hat{\uv} = &\argmax_{\uv} P(\uv|\mathsf{X},\Yv) \\
        =&\argmax_{\uv} \big(\frac{p}{1-p}\big)^{\sum_{j=1}^{n} u_{j}} \\
        =&\argmax_{\uv} \log\big(\frac{p}{1-p}\big)\sum_{j=1}^{n} u_{j} \\
        =&\argmin_{\uv} \sum_{j=1}^{n} u_{j}.
    \end{aligned}
    \label{lp_argmin_noiseless}
\end{equation}

\section{MORE DETAILS ON IMBALANCED EXAMPLE}

Combining these conditions and using notation \eqref{eq:imbal_nu_star}, we have
the following simplication of \eqref{eq:rate_imbal_linear_k2}:
\[
    \lim_{n \to \infty}
    \frac{\log_2 |\Sc|}{t} = 
    \begin{cases}
    % \max_{\nu > 0} 
        \frac{H_2\left(e^{-(1-\gamma) \nu^*}\right)}
             {e^{ \gamma \nu^*} } 
             \left(1 + \frac{\gamma}{1-\gamma} \frac{c - \theta}{1-\theta} \right) 
             & \text{ if }
             \frac{c-\theta}{1-\theta} \le
             \left(\frac{1-\gamma}{\gamma} \right)
             \left(
              H_2\left(e^{-\nu^*}\right) 
              \frac{ e^{ \gamma \nu^*} }{ H_2\left(e^{-(1-\gamma) \nu^*}\right) }
              - 1
             \right)
            %   \frac{H_2\left(e^{-(1-\gamma) \nu^*}\right)}
            %  {e^{ \gamma \nu^*} } 
            %  \left(1 + \frac{\gamma\left(c - \theta \right)}{(1-\gamma)(1-\theta)} \right)
            %  \le
            %  H_2\left(e^{-\nu^*}\right)
     \\ 
     \\
      1  & \text{ if } 
     \frac{c-\theta}{1-\theta} \ge
      \left(\frac{1-\gamma}{\gamma}\right)
     \left(\frac{2^{\gamma}}{H_2\left(2^{-(1-\gamma)}\right)} - 1 \right)
         %  1 \le 
    %      \frac{H_2\left(2^{-(1-\gamma)}\right)}{2^{\gamma} } 
    %      \left(1 + \frac{\gamma\left(c - \theta \right)}{(1-\gamma)(1-\theta)} \right) 
                 \\
             \\
     \text{as in } \eqref{eq:rate_imbal_linear_k2} & \text{ otherwise.}
    \end{cases}
\]
which we plot in Figure~\ref{fig:limits_imbalanced}.
\begin{figure}[htbp!]
    \centerline{\includegraphics[width = 8cm]{limit_imbalanced_gamma.png}}
\caption{Limits as defined in \eqref{eqn: limit S} for various $\gamma$ and ratio $\frac{c - \theta}{1-\theta}$. {\bf \color{blue} [TODO: Check if the assumption of Corollary 2.10 holds for everything plotted]}}
\label{fig:limits_imbalanced}
\end{figure}
Likewise, we have
\begin{equation}
\label{eq:imbalance_limit_n_chooose_k}
    \lim_{n \to \infty}
    \frac{\log_2 \binom{n}{k}}{t} = 
    \max_{\nu > 0} \,
        \min\left\{
        H_2(e^{-\nu}) \frac{1-\theta}{(1-\theta) - \gamma(1-c)}, \,
        \frac{H_2\left(e^{-(1-\gamma) \nu}\right)}
             {\left(1-\gamma\right) e^{ \gamma \nu} } 
        \right\},
\end{equation}
and similar analysis as above gives us
\[
    \lim_{n \to \infty}
    \frac{\log_2 \binom{n}{k}}{t} = 
    \begin{cases}
        \frac{H_2\left(e^{-(1-\gamma) \nu^*}\right)}
             {e^{ \gamma \nu^*} } 
             \left( \frac{1}{1-\gamma} \right) 
             & \text{ if }
             \frac{c-\theta}{1-\theta} \le
             \left(\frac{1-\gamma}{\gamma} \right)
             \left(
              H_2\left(e^{-\nu^*}\right) 
              \frac{ e^{ \gamma \nu^*} }{ H_2\left(e^{-(1-\gamma) \nu^*}\right) }
              - 1
             \right)
            %   \frac{H_2\left(e^{-(1-\gamma) \nu^*}\right)}
            %  {e^{ \gamma \nu^*} } 
            %  \left(1 + \frac{\gamma\left(c - \theta \right)}{(1-\gamma)(1-\theta)} \right)
            %  \le
            %  H_2\left(e^{-\nu^*}\right)
          \\
          \\
          \frac{1-\theta}{(1-\theta) - \gamma(1-c)}  & \text{ if } 
             \frac{c-\theta}{1-\theta}
           \ge
          \left(\frac{1-\gamma}{\gamma}\right)
         \left(\frac{2^{\gamma}}{H_2\left(2^{-(1-\gamma)}\right)} - 1 \right)
          \\
         \\
      \text{as in \eqref{eq:imbalance_limit_n_chooose_k}} & \text{ otherwise,}
    \end{cases}
\]
{\bf \color{red} [TODO (Ivan): I think there is an issue with the order of operations.  Finding a single $\nu$ that makes both $t$ terms small is ``harder'' than finding separate $\nu$ for the two.  We might need to just set $\nu = \ln 2$ and give a sufficient condition under which a ``rate'' of $1$ is attained.  Then we might need to reproduce Figure 4 with a proper numerical optimization over $\nu$ (I think the curves will be smoother).]}
which shows {\bf \color{red} [TODO (Ivan): Second term isn't immediately clear]} that the required $t$ is fewer than $\log_2 \binom{n}{k}$, and so fewer than the required number of tests in the absence of prior information (see Lemma~\ref{lem:standard_bounds}) 
{\bf \color{magenta} [Response (Ivan): I think it is messy to prove the third one is bigger than 1, maybe show through plot?]}.

    % Denoting the resulting value by $t_1$, 
    % We denote the maximizing $\nu$ by $\nu^*$:
    %  The limit as defined in \eqref{eqn: limit S} is
    %  with $t_1$ in place of $t$) is
    % \begin{equation}
    % \label{eq:imbal_nu_star}    
    % \nu^*
    %     \coloneqq
    %     \argmax_{\nu > 0} f_2(\nu) =
    %     \argmax_{\nu > 0} 
    %     \frac{H_2\left(e^{-(1-\gamma) \nu}\right)}
    %          {e^{ \gamma \nu} } 
    %          \left(1 + \frac{\gamma\left(c - \theta \right)}{(1-\gamma)(1-\theta)} \right).
    % \end{equation}
    % Similar to the case for $f_1$, if 
    % \[
    %     f_2\left(\nu^*\right) \le  f_1\left(\nu^*\right)
    % \]
    %
    % Then the limit as defined in \eqref{eqn: limit S} is
    % \[
    %     \frac{H_2\left(e^{-(1-\gamma) \nu^*}\right)}
    %          {e^{ \gamma \nu^*} } 
    %          \left(1 + \frac{\gamma}{1-\gamma} \frac{c - \theta}{1-\theta} \right)
    % \]

% The second maximand is minimized at $\nu = \ln 2$,
% and the limits as defined in \eqref{eqn: limit S} and \eqref{eqn: limit n c k}  are
% \[
%     \lim_{n \to \infty}
%     \frac{\log_2 |\Sc|}{t} = 
%     \frac{\left( (1-\theta) - \gamma(1-c) \right) \left(k \log_2 n \right)}{t} \left( 1 +o(1) \right)
%     = 1 +o(1)
% \]
% and
% \[
%     \lim_{n \to \infty}
%     \frac{\log_2 \binom{n}{k}}{t} = 
%     \frac{ (1-\theta)   \left(k \log_2 n \right)}{t} \left( 1 +o(1) \right)
%     = \frac{1-\theta}{(1-\theta) - \gamma(1-c)} \left(1 +o(1) \right).
% \]
% For the first maximand, we can show by differentiation that,
% (similar to \eqref{eq:card_bound_optimal_nv},) the minimizing $\nu$  satisfies
% \[
%     H_2\left(e^{-(1-\gamma) \nu}\right) =
%     (\gamma - 1) \log_2 \left(1- e^{-(1-\gamma) \nu}\right),
% \]
% which appears to have no closed-form solution for a general $\gamma$.
% The numerically minimized $\nu$ is expected to be similar to the one shown in Figure~\ref{img: optimal nu}.
% The limits as defined in \eqref{eqn: limit S} and \eqref{eqn: limit n c k}  are
% \[
%     \lim_{n \to \infty}
%     \frac{\log_2 |\Sc|}{t} = 
%     \max_{\nu > 0} 
%     \frac{H_2\left(e^{-(1-\gamma) \nu}\right)}
%          {(1-\gamma)  \left(e^{ \gamma \nu} \right)} 
%          \frac{(1-\theta) - \gamma(1-c)}{1-\theta}  =
%     \max_{\nu > 0} 
%     \frac{H_2\left(e^{-(1-\gamma) \nu}\right)}
%          {e^{ \gamma \nu} } 
%          \left(1 + \frac{\gamma}{1-\gamma} \frac{c - \theta}{1-\theta} \right)
% \]
% and
% \[
%      \lim_{n \to \infty}
%     \frac{\log_2 \binom{n}{k}}{t} = 
%     \max_{\nu > 0} 
%     \frac{H_2\left(e^{-(1-\gamma) \nu}\right)}
%          {(1-\gamma)  \left(e^{ \gamma \nu} \right)}. 
% \]

==> app0.tex <==
\subsubsection{Linear Programming}
\begin{defn}
A linear program (LP) is the problem of optimizing a linear function over a polyhedron:
\[
\begin{aligned}
    &\min_{\mathbf{x} \in \RR^{n}} \mathbf{c}^{T}\mathbf{x} \\
    \text{subject to } &\mathsf{A}\mathbf{x} \leq \mathbf{b} \\
    & \mathbf{x} \geq \mathbf{0}, 
\end{aligned}
\]
where $\mathsf{A} \in \RR^{m \times n}$ and $\mathbf{b} \in \RR^{m}$ in the case of $n$ variables and $m$ constraints.
\label{lp_def}
\end{defn}
Here the $\mathbf{x}$ is the variable to be determined, $ \mathbf{c}$ and $\mathbf{b}$ are given vectors, and $\mathsf{A}$ is a given matrix. The function whose value is to be maximized or minimized ($\mathbf{c}^{T}\mathbf{x}$ in this case) is called the objective function. The inequalities $\mathsf{A}\mathbf{x} \leq \mathbf{b}$ and $\mathbf{x} \geq \mathbf{0}$ are the constraints which specify a convex polytope over which the objective function is to be optimized.


\subsubsection{Quadratic Programming}
\begin{defn}
A quadratic programming (QP) is an optimization problem with a quadratic objective and linear constraints
\[
\begin{aligned}
    &\min_{\mathbf{x} \in \RR^{n}} \mathbf{x}^{T}\mathsf{Q}\mathbf{x} + \mathbf{q}^{T}\mathbf{x} + c \\
    \text{subject to } &\mathsf{A}\mathbf{x} \leq \mathbf{b},
\end{aligned}
\]
where, $\mathsf{Q} \in \RR^{n \times n}$ is a real symmetrical matrix, $\mathbf{q} \in \RR^{n}$, $c \in \RR$, $\mathsf{A} \in \RR^{m \times n}$, and $\mathbf{b} \in \RR^{m}$.
\label{qp_def}
\end{defn}
The difficulty of QP changes drastically depending on whether the adjacency matrix $\mathsf{Q}$ is positive semidefinite (PSD) or not. When $\mathsf{Q}$ is PSD, the problem is called a convex QP. When non-convexities are present, however, things become much more difficult. Convex QP is generally much easier to solve than non-convex one, except for the situations where the optimized vectors need to take on integer values, which leads to the formulation of a mixed-integer quadratic programming (MIQP) problem.
